Measurement of the $\Omega_c^0$ baryon lifetime

We report a measurement of the lifetime of the $\Omega_c^0$ baryon using proton-proton collision data at center-of-mass energies of 7 and 8~TeV, corresponding to an integrated luminosity of 3.0 fb$^{-1}$ collected by the LHCb experiment. The sample consists of about 1000 $\Omega_b^-\to\Omega_c^0\mu^-\bar{\nu}_{\mu} X$ signal decays, where the $\Omega_c^0$ baryon is detected in the $pK^-K^-\pi^+$ final state and $X$ represents possible additional undetected particles in the decay. The $\Omega_c^0$ lifetime is measured to be $\tau_{\Omega_c^0} = 268\pm24\pm10\pm2$ fs, where the uncertainties are statistical, systematic, and from the uncertainty in the $D^+$ lifetime, respectively. This value is nearly four times larger than, and inconsistent with, the current world-average value.

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}


==> justification.tex <==
\section*{Justification}

This paper presents a new measurement of the charm baryon lifetime using
a sample of about 1000 $\Omegac$ baryons, observed through semileptonic
$\Omegab\to\Omegac\mun\neumb X$ decays. This sample is about 10 times larger than used for any previous measurement of the $\Omegac$ lifetime. The measured lifetime of $\tau_{\Omegac}=268\pm24\pm10\pm2$~fs
 is about four times larger than, and inconsistent with,  
the world average value of $69\pm12$~fs. This result may lead to a rethinking of the relative size of various spectator and non-perturbative effects in hadrons containing heavy quarks.


%\vspace{1.0in}

%Estimated word count:

%Text:     3215

%1 Table:   78

%Eqs:      96

%Figures   310

%--------------

%Total:    3699


==> titleAndAbstractPlainText.tex <==
Measurement of the $\Omega_c^0$ baryon lifetime


We report a measurement of the lifetime of the $\Omega_c^0$ baryon
using proton-proton collision data at center-of-mass energies of 7 and 8~TeV, corresponding to an 
integrated luminosity of 3.0 fb$^{-1}$ collected by the 
LHCb experiment. The sample
consists of about 1000 $\Omega_b^-\to\Omega_c^0\mu^-\bar{nu} X$ signal decays, where the $\Omega_c^0$ baryon is detected in the
$pK^-K^-\pi^+$ final state and $X$ represents possible additional undetected particles in the decay.
The $\Omegac$ lifetime is measured to be $\tau_{\Omega_c^0} = 268\pm24\pm10\pm2$ fs, where the uncertainties 
are statistical, systematic, and from the uncertainty in the $\Dp$ lifetime, respectively.
This value is nearly four times larger than, and inconsistent with, the current world-average value.

